The Landscape of Compute-near-memory and Compute-in-memory: A Research and Commercial Overview

In today's data-centric world, where data fuels numerous application domains, with machine learning at the forefront, handling the enormous volume of data efficiently in terms of time and energy presents a formidable challenge. Conventional computing systems and accelerators are continually being pushed to their limits to stay competitive. In this context, computing near-memory (CNM) and computing-in-memory (CIM) have emerged as potentially game-changing paradigms. This survey introduces the basics of CNM and CIM architectures, including their underlying technologies and working principles. We focus particularly on CIM and CNM architectures that have either been prototyped or commercialized. While surveying the evolving CIM and CNM landscape in academia and industry, we discuss the potential benefits in terms of performance, energy, and cost, along with the challenges associated with these cutting-edge computing paradigms.

==> abbrev.tex <==
\acro{ap}[AP]{\emph{access port}}
\acro{afd}[AFD]{\emph{access frequency based distribution}}
\acro{ab}[AB]{\emph{alternation base}}
\acro{ac}[AC]{\emph{alternation candidate}}
\acro{af}[AF]{\emph{antiferromagnetically}}
\acro{bb}[BB]{\emph{basic block}}
\acro{blo}[BLO]{\emph{bi-directional linear ordering}} 
\acro{am}[AM]{\emph{associative memory}}
\acro{api}[API]{\emph{application programming interface}}
\acro{cpu}[CPU]{\emph{central processing unit}}
\acro{ctl}[CTL]{\emph{chemical templating layers}}
\acro{cst}[CST]{\emph{chiral spin torque}}
\acro{cw}[CW]{\emph{clockwise}}
\acro{cim}[CIM]{\emph{computing in memory}}
\acro{cfg}[CFG]{\emph{control flow graph}}
\acro{cnn}[CNN]{\emph{convolutional neural network}}
\acro{ccw}[CCW]{\emph{counterclockwise}}
\acro{dpu}[DPU]{\emph{data processing unit}}
\acro{date}[DATE]{\emph{Design, Automation and Test in Europe}}
\acro{dma}[DMA]{\emph{disjoint memory accesses}}
\acro{dsl}[DSL]{\emph{domain specific language}}
\acro{dw}[DW]{\emph{domain wall}}
\acro{dbc}[DBC]{\emph{domain wall block cluster}}
\acro{dwm}[DWM]{\emph{domain wall memory}}
\acro{dram}[DRAM]{\emph{dynamic random access memory}}
\acro{dmi}[DMI]{\emph{Dzyaloshinskii-Moriya interaction}}
\acro{ec}[EC]{\emph{error correction}}
\acro{ecc}[ECC]{\emph{error correction code}}
\acro{ed}[ED]{\emph{error detection}}
\acro{ect}[ECT]{\emph{exchange coupling torque}}
\acro{fefet}[FeFET]{\emph{ferroelectric field effect transistor}}
\acro{feram}[FeRAM]{\emph{ferroelectric RAM}}
\acro{fpga}[FPGA]{\emph{field-programmable gate array}}
\acro{ftj}[FTJ]{\emph{ferroelectric tunnel junction}}
\acro{ga}[GA]{\emph{genetic algorithm}}
\acro{gemm}[GEMM]{\emph{general matrix-matrix multiplication}}
\acro{gmr}[GMR]{\emph{giant-magnetoresistance}}
\acro{gpu}[GPU]{\emph{graphical processing unit}}
\acro{hw}[HW]{\emph{hardware}}
\acro{hdd}[HDD]{\emph{hard disk drive}}
\acro{hdc}[HDC]{\emph{hyperdimensional computing}}
\acro{hdcr}[HDCR]{\emph{HyperDimensional Computing in Racetrack}}
\acro{hv}[HV]{\emph{hypervector}}
\acro{iga}[IGA]{\emph{improved genetic algorithm}}
\acro{ilp}[ILP]{\emph{integer linear programming}}
\acro{inlp}[INLP]{\emph{integer nonlinear programming}}
\acro{iot}[IoT]{\emph{internet of things}}
\acro{islped}[ISLPED]{\emph{International Symposium on Low Power Electronics and Design}}
\acro{im}[IM]{\emph{item memory}}
\acro{lr}[LR]{\emph{language recognition}}
\acro{llc}[LLC]{\emph{last level cache}}
\acro{lut}[LUT]{\emph{lookup table}}
\acro{mram}[MRAM]{\emph{magnetic RAM}}
\acro{mtj}[MTJ]{\emph{magnetic tunnel junction}}
\acro{mm}[MM]{\emph{matrix multiplication}}
\acro{mwhp}[MWHP]{\emph{maximum weighted Hamiltonian path}}
\acro{mwhpc}[MWHPC]{\emph{maximum weighted Hamiltonian path cover}}
\acro{mttf}[MTTF]{\emph{mean time to failure}}
\acro{mrc}[MRC]{\emph{multilane racetrack cache}}
\acro{mlc}[MLC]{\emph{multi level cell}}
\acro{mlir}[MLIR]{\emph{multi level intermediate representation}}
\acro{npu}[NPU]{\emph{neural processing unit}}
\acro{ndp}[NDP]{\emph{near data processing}}
\acro{nmc}[NMC]{\emph{near memory computing}}
\acro{nvm}[NVM]{\emph{nonvolatile memory}}
\acro{ofu}[OFU]{\emph{order of first use}}
\acro{occ}[OCC]{\emph{open CIM compiler}}
\acro{pte}[PTE]{\emph{page table entry}}
\acro{pcm}[PCM]{\emph{phase change memory}}
\acro{pma}[PMA]{\emph{perpendicular magnetic anisotropy}}
\acro{pg}[PG]{\emph{processing group}}
\acro{pim}[PIM]{\emph{processing in memory}}
\acro{pc}[PC]{\emph{program counter}}
\acro{rtm}[RTM]{\emph{racetrack memory}}
\acro{rm}[RM]{\emph{racetrack memory}}
\acro{ram}[RAM]{\emph{random access memory}}
\acro{rw}[RW]{\emph{random walk}}
\acro{re}[RE]{\emph{rare earth}}
\acro{reram}[ReRAM]{\emph{resistive RAM}}
\acro{spm}[SPM]{\emph{scratchpad memory}}
\acro{shrimp}[SHRIMP]{\emph{shift-reducing instruction memory placement}}
\acro{soa}[SOA]{\emph{single offset assignment}}
\acro{sw}[SW]{\emph{software}}
\acro{ssd}[SSD]{\emph{solid state drive}}
\acro{sot}[SOT]{\emph{spin-orbit torque}}
\acro{stt}[STT]{\emph{spin-transfer torque}}
\acro{scop}[SCoP]{\emph{static control part}}
\acro{sram}[SRAM]{\emph{static random access memory}}
\acro{sts}[STS]{\emph{sub threshold shift}}
\acro{saf}[SAF]{\emph{synthetic antiferromagnetic}}
\acro{tpu}[TPU]{\emph{tensor processing unit}}
\acro{taco}[TACO]{\emph{Transactions on Architecture and Code Optimization}}
\acro{tm}[TM]{\emph{transition metal}}
\acro{tr}[TR]{\emph{transverse read}}
\acro{trd}[TRD]{\emph{transverse read distance}}
\acro{tmr}[TMR]{\emph{tunneling magnetoresistance}}
\acro{tw}[TW]{\emph{transverse write}}
\acro{vt}[VT]{\emph{Varshamov-Tenengolts}}
\acro{vnand}[V-NAND]{\emph{vertical NAND}}

==> contents/ai-accel.tex <==
This section shows AI accelerators' technology and market trends (including but not limited to CIM/CNM).

\begin{figure}[tbh]
\centering
\includegraphics[scale=0.2]{figures/Nvidia-vs-AMD-vs-Intel_AI-Chip-Sales.jpeg}
%\vspace{-0.4cm}
\caption{AI chips sales comparison of various companies (source: Visualcapitalists).} 
\label{fig:AI-chips-sales}
%\vspace{-0.4cm}
\end{figure}


\begin{figure}[tbh]
\centering
\includegraphics[scale=0.2]{figures/AI-accel.png}
%\vspace{-0.4cm}
\caption{Comparison of various AI accelerators~\cite{kendall2020building}.} 
\label{fig:AI-accel}
%\vspace{-0.4cm}
\end{figure}


\begin{figure}[tbh]
\centering
\includegraphics[scale=0.2]{figures/AI-accel.png}
%\vspace{-0.4cm}
\caption{Comparison of various AI accelerators~\cite{kendall2020building}.} 
\label{fig:AI-accel}
%\vspace{-0.4cm}
\end{figure}

\begin{figure}[tbh]
\centering
\includegraphics[scale=0.2]{figures/memristors-advancements.png}
%\vspace{-0.4cm}
\caption{Advancements in memristors. Left: Breakthroughs in memristors functionalities, Right: developments timeline~\cite{zidan2018future}.} 
\label{fig:memristors-adv}
%\vspace{-0.4cm}
\end{figure}

\begin{figure}[tbh]
\centering
\includegraphics[scale=0.2]{figures/perf-vs-power-AI-accel.png}
%\vspace{-0.4cm}
\caption{Performance and power comparison of various publicly announced AI accelerators~\cite{ai-accel-review-22}.} 
\label{fig:AI-accel-trends}
%\vspace{-0.4cm}
\end{figure}


==> contents/terminology.tex <==
This section highlights the bottleneck in the Von Neumann computing model by discussing its working mechanism, motivates the need for memory-centric computing, and explains the terminology. 

\subsection{Mainstream Von-Neumann Computing}
\label{subsec:vonNeumann}
The Von Neumann computation model stands as the most widespread and accomplished model to date. It encompasses four primary components: the \ac{cpu}; the memory, responsible for retaining both program instructions and data; the storage unit, and the interconnect, facilitating the bidirectional transmission of data and instructions between the \ac{cpu} and memory. The \ac{cpu} consists of compute units, referred to as ALU or FPU, responsible for performing logic and arithmetic operations as well as a control unit that controls the flow of execution. An important component of the control unit is the \ac{pc} that controls the flow of addressable instructions. To execute an instruction, the Von Neumann model follows a structured sequence of operations which are listed (in their order of execution) below. 

\begin{itemize}
    \item Fetch instruction: The control unit fetches the next instruction from the memory using the PC as a reference and store it in a register.

    \item Execute instruction: The instruction is executed 
    by compute units in the \ac{cpu} depending on the operation. This step may involve performing arithmetic calculations, logical comparisons, or other data manipulations.
    If the instruction requires accessing memory, e.g., $f(D)$ in Figure~\ref{fig:von-Neumann} requires $D$, it is fetched from the memory. 
    After executing the instruction, the state of the machine may change, e.g., Result $f(D)$ in Figure~\ref{fig:von-Neumann}.

    \item Update Program Counter: After the instruction is executed, the PC is updated to point to the next instruction in memory and the same cycle repeats for the next instruction.
\end{itemize}

\begin{figure}[tbh]
\centering
\includegraphics[scale=0.1]{figures/von-neumann.png}
%\vspace{-0.4cm}
\caption{A simplified view of the Von Neumann architecture~\cite{cim_survey}} 
\label{fig:von-Neumann}
%\vspace{-0.4cm}
\end{figure}

As depicted in Figure~\ref{fig:von-Neumann}, the interaction between memory and the processor in the Von Neumann architecture is facilitated through address and data buses (shown with different colours). However, because \ac{cpu} performance significantly outpaces memory performance (as illustrated in Figure~\ref{fig:memwall}), the Von Neumann models are often bottlenecked by the memory. To address this challenge and mitigate the impact of larger memory access latencies on the \ac{cpu}, modern processors incorporate a tiered hierarchy of caches. Caches are smaller memory units that, while being much smaller compared to main memory and storage, are notably faster. The first-level cache (L1) is typically integrated onto the \ac{cpu} chip and operates nearly at \ac{cpu} speed, enabling single-cycle access. L2 cache is usually shared by multiple cores and can vary in location depending on the design goals. Some systems even include an L3 cache, usually larger and situated off-chip.

Note that Von Neumann architectures are characterized by the sequential execution of instructions. However, in multi-core \ac{cpu} systems, parallel execution of instructions at various levels of granularity, including instruction-level, data-level, and thread-level parallelisms, is supported. To enhance performance and energy efficiency in resource-constrained systems, specialized accelerators are often developed and integrated on the same chip. For instance, in application domains such as embedded systems, digital signal processing, and networking, \ac{mpsoc} architectures are employed. These integrate multiple processor cores, memory, input/output interfaces, and potentially specialized hardware accelerators, enabling parallel execution of different tasks to meet specific constraints. 

Although these designs may significantly enhance performance when compared to conventional \ac{cpu}-only systems, the underlying design principle remains \ac{cpu}-centric and follows the Von Neumann model of execution. Consequently, the performance improvements, largely resulting from concurrent execution, heavily rely on the nature of the application. In cases where an application is memory-bound, i.e., most of the execution time is spend on the memory accesses and not on the actual compute operations, the shared data bus is fully occupied and becomes a bottleneck. Even for compute-bound applications, where these architectures can yield substantial gains in execution time, power consumption remains largely unaffected and might even increase due to the complex structure of these systems\hf{Not sure about the last sentence?}.

%% Another resource for terminology: https://dl.acm.org/doi/pdf/10.1145/3566097.3568356

\subsection{Memory-centric computing}
\label{subsec:mem-centric}
Unlike conventional computing systems where \ac{cpu} has a central role and is responsible for all computations, most computations in the memory-centric designs are performed within or near memory. 
As depicted in Figure~\ref{fig:mem-centric}, the core concept revolves around minimizing data transfer on the bus by relocating a substantial share of computations closer to the data (memory). The \ac{cpu}'s primary role becomes issuing commands and handling computations that cannot be effectively executed in close proximity to the memory.

The concept of memory-centric computing is not a novel one, but it has experienced a significant surge in recent years. Consequently, various terms have emerged, often referring to the same idea, and more detailed classifications have been introduced in architectural designs. 
This section aims to clarify the terminology surrounding these approaches.

\begin{figure}[tbh]
\centering
\includegraphics[scale=0.11]{figures/mem-centric.png}
%\vspace{-0.4cm}
\caption{(a) Conventional computing system where an operation $f$ is performed on data $D$ in the \ac{cpu} (b) Memory-centric design where $f$ is computed in the proximity of $D$ and \ac{cpu} is mainly working as a control unit~\cite{cim_survey}.} 
\label{fig:mem-centric}
%\vspace{-0.4cm}
\end{figure}
Computing systems can be broadly divided into two categories: \acf{cim} systems and \ac{com} systems (see Section~\ref{subsec:vonNeumann}).
In the literature, there are different names for similar things. These architectures are often named based on (1) the \emph{location} of the compute units within the memory hierarchy ( near cache or near main memory), or (2) based on the underlying paradigm, i.e., whether the memory device itself is used to implement computation (\ac{cim}), or whether extra CMOS-logic \hf{CMOS here is the first time} is added near the memory to perform computations (\ac{cnm}). 
\ac{cim} systems are also frequently referred to as \ac{imc}, \ac{imp}, \ac{pim}, \ac{pum} or \ac{lim} systems~\cite{LiM}. For the purposes of this report, we will use the term \ac{cim}. 

\begin{figure}[tbh]
\centering
\includegraphics[scale=0.13]{figures/SiP.png}
%\vspace{-0.4cm}
\caption{System Architecture~\cite{delft-cim-survey}} 
\label{fig:SiP}
%\vspace{-0.4cm}
\end{figure}

To explain this further, let us consider a high-level overview of a memory system in a package, as depicted in Figure~\ref{fig:SiP}.
A compute operation can be a logic operation or an arithmetic operation such as addition and multiplication. When operations are computed outside the memory (\ac{com}) using conventional computing cores (\textcircled{\raisebox{-0.09em}{4}} in the figure), the architecture is a conventional Von Neumann system (see Section~\ref{subsec:vonNeumann}). On the other hand, if the computations are performed outside the memory but with a dedicated logic unit connected to the memory module via a high-bandwidth channel (\textcircled{\raisebox{-0.09em}{3}} in the figure), the system is referred to as a \acf{cnm} or \ac{nmc} or \ac{nmp}, or \ac{pnm} system. In this report, we will restrict ourselves to calling it \ac{cnm}.

In the \ac{cim} category, computations can be carried out using memory cells within the memory array, known as \ac{cim-a} (see (\textcircled{\raisebox{-0.09em}{1}} in the figure). Alternatively, computations can occur in the memory peripheral circuitry, termed \ac{cim-p} \textcircled{\raisebox{-0.09em}{2}} in the figure). Figure~\ref{fig:cim-cnm-com} provides a high-level architectural comparison illustrating the distinctions between \ac{cim}, \ac{cnm}, and \ac{com} architectures.

\begin{figure}[tbh]
\centering
% \includegraphics[scale=0.13]{figures/cim-cnm-com.png}
\includegraphics[scale=0.13]{figures/COM-CNM-CIM-wo-dots.png}

%\vspace{-0.4cm}
\caption{High-level overview of COM (mainstream computing), \ac{cnm} (where logic is integrated on the memory modules), and \ac{cim} architectures (where the memory performs computations and stores data)~\cite{mram-review}.} 
\label{fig:cim-cnm-com}
%\vspace{-0.4cm}
\end{figure}

In \ac{cim-a}, memory cells are often modified to support logic design, e.g., in~\cite{magic}. Sometimes, it also necessitates changes to the periphery to support the modified cells. Therefore, some literature further divides the \ac{cim-a} designs into basic \ac{cim-a} that do not require any modifications to the periphery, e.g.,~\cite{sf-logic}, and hybrid \ac{cim-a} that requires support from the peripheral circuit.  A well-known example of a hybrid \ac{cim-a} is the MAGIC design~\cite{magic} that requires extending the peripheral circuit to write multiple memory rows simultaneously. 

Typical examples of \ac{cim-p} architectures are crossbars employing \acp{adc} and \acp{dac} to implement vector-matrix multiplication and other logic operations~\cite{prime, isaac}. Additionally, \ac{cim-p} designs employing customized sense amplifiers also exist~\cite{li2016pinatubo}. Similar to \ac{cim-a}, \ac{cim-p} can also be basic (e.g., ~\cite{li2016pinatubo}), requiring no changes to the memory array, as well as hybrid (e.g., ~\cite{isaac}). A summary of the terminology's classification is presented in Figure~\ref{fig:term}.

Both \ac{cim-a} and \ac{cim-p} can also be used together, wherein the memory array calculates partial results that are later post-processed or accumulated in the peripheral circuit.  In such cases, it is referred to as a \ac{cim} architecture.

\begin{figure*}[tbh]
\centering
\includegraphics[scale=0.5]{figures/terminology.pdf}
%\vspace{-0.4cm}
\caption{\ac{cim} and \ac{cnm} classification.} 
\label{fig:term}
%\vspace{-0.4cm}
\end{figure*}

